Who Thinks First? Designing Productive Friction with Engage-to-Unlock GenAI

Generative AI can support writing, but frictionless access may cause cognitive offloading before users develop their own ideas. We introduce Engage-to-Unlock, a productive-friction mechanism that unlocks generative capabilities after users meaningfully engage with the task. In a controlled experiment (N = 398), participants completed a writing task under one of four conditions: Human-Only, Standard Chatbot, Engage-to-Unlock, or Time-Matched Unlock, which matched unlock timing to Engage-to-Unlock participants but independent of users' engagement, then evaluated passages for evidence and inferential errors. Results show that Engage-to-Unlock redistributed effort across tasks: participants spent more time writing and less time evaluating, without increasing overall task duration. They also submitted more prompts than in other AI-assisted conditions and showed the highest accuracy-per-time evaluation efficiency across conditions. These findings suggest that designing GenAI access to encourage early human engagement may provide a productive form of friction, while retaining active AI use and efficient downstream evaluation.

==> meta/authors.tex <==
% Paper authors and affiliations.
\makeatletter
\@ifclassloaded{googledeepmind}{%
  \author[1,2]{Xiaotian Su}
  \author[1]{Laura Rimell}
  \author[1,3]{Jiazheng Li}
  \author[1]{Amal Rannen-Triki}
  \author[1]{Ulrich Paquet}   
  \author[1]{Lisa Anne Hendricks}    
  \author[5]{Rida Qadri} 
  \author[6]{Daphne Ippolito}
  \author[1]{Piotr Mirowski}

  \affil[1]{Google DeepMind, London, UK}
  \affil[2]{Computer Science, ETH Zurich, Zurich, Switzerland}
  \affil[3]{King's College London, London, UK}
  \affil[5]{Google Research, San Francisco, California, USA}
  \affil[6]{Google DeepMind, Mountain View, California, USA}
}{%
  \author{Xiaotian Su}
  \email{xiaotian.su@inf.ethz.ch}
  \email{xiaotiansu@google.com}
  \affiliation{%
    \institution{ETH Zurich}
    \city{Zurich}
    \country{Switzerland}}
  \affiliation{%
    \institution{Google DeepMind}
    \city{London}
    \country{UK}}

  \author{Laura Rimell}
  \email{laurarimell@google.com}
  \affiliation{%
    \institution{Google DeepMind}
    \city{London}
    \country{UK}}

  \author{Jiazheng Li}
  \email{jiazheng.li@kcl.ac.uk}
  \affiliation{%
    \institution{King's College London}
    \city{London}
    \country{UK}}

  \author{Amal Rannen-Triki}
  \email{arannen@google.com}
  \affiliation{%
    \institution{Google DeepMind}
    \city{London}
    \country{UK}}

  \author{Ulrich Paquet}
  \email{upaq@google.com}
  \affiliation{%
    \institution{Google DeepMind}
    \city{London}
    \country{UK}}

  \author{lmh}
  \email{lmh@google.com}
  \affiliation{%
    \institution{Google}
    \city{London}
    \country{UK}}

  \author{Google Research Author}
  \affiliation{%
    \institution{Google Research}
    \city{San Francisco}
    \state{California}
    \country{USA}}

  \author{Daphne I.}
  \email{dei@google.com}
  \email{daphnei@seas.upenn.edu}
  \email{daphnei@cmu.edu}
  \affiliation{%
    \institution{Google DeepMind}
    \city{Mountain View}
    \state{California}
    \country{USA}}
  \affiliation{%
    \institution{University of Pennsylvania}
    \city{Philadelphia}
    \state{Pennsylvania}
    \country{USA}}
  \affiliation{%
    \institution{Carnegie Mellon University}
    \city{Pittsburgh}
    \state{Pennsylvania}
    \country{USA}}

  \author{Piotr Mirowski}
  \email{piotrmirowski@google.com}
  \affiliation{%
    \institution{Google DeepMind}
    \city{London}
    \country{UK}}

  \renewcommand{\shortauthors}{Su et al.}
}
\makeatother

